Responsibility in Actor-Based Systems

The enormous growth of the complexity of modern computer systems leads to an increasing demand for techniques that support the comprehensibility of systems. This has motivated the very active research field of formal methods that enhance the understanding of why systems behave the way they do. One important line of research within the verification community relies on formal notions that measure the degree of responsibility of different actors. In this paper, we first provide a uniform presentation of recent work on responsibility notions based on Shapley values for reactive systems modeled by transition systems and considering safety properties. The paper then discusses how to use these formal responsibility notions and corresponding algorithms for three different types of actor sets: the module-based notion serves to reason about the impact of system components on the satisfaction or violation of a safety property. Responsibility values for value-based actor sets and action-based actors allow for the identification of program instructions and control points that have the most influence on a specification violation. Beyond the theoretical considerations, this paper reports on experimental results that provide initial insights into applicability and scalability.

==> 05-complexity.tex <==
\section{Algorithms and complexity}
\label{sec:complexity}

To determine the complexity of computing backward responsibility, two decision problems and one computation problem are defined in \cite{BackwardResponsibility}. In the \emph{positivity problem}, the question is whether the responsibility of a given agent is positive. In the \emph{threshold problem}, the question is whether the responsibility of a given agent is greater than or equal to a given threshold. In the \emph{responsibility computation problem}, the goal is to compute the responsibility of a given state.

The Shapley value is defined as a sum over all coalitions $C \subseteq \actors$. As the number of such coalitions is exponential in the number of actors and checking each coalition only requires polynomial runtime, a na\"ive implementation can compute responsibility in exponential time (and one can show that this is possible with polynomial space).

In \cite{BackwardResponsibility}, complexity bounds are given for the case whether every actor is a singleton. They show that no efficient, polynomial algorithm exists for these problems: The positivity problem is NP-complete, the threshold problem is NP-hard and the computation problem is \#P-hard.

While they only considers singleton actors, the results can easily be generalised to other actor sets as well. Because singleton actors are a subset of all actor sets, the general problems must be at least as hard as the single-actor problems. Additionally, the na\"ive algorithm used to show inclusion in NP and PSPACE can easily be extended to support non-singleton actors.

While the asymptotic complexity remains unchanged, supporting non-singleton actors nonetheless deliver a major performance improvement: The number of coalitions that need to be checked is exponential \emph{in the number of actors}. By using non-singleton actors, the number of actors is decreased and therefore, models that were previously too large to analyse may become tractable. For example, a simple program with a program counter and a few other variables may produce a transition system with $100$ states. Computing individual responsibility requires requires analysis of roughly $2^{100}$ coalitions, which is intractable. On the other hand, if we create actors for each value of the program counter and if the program counter has $20$ values, the number of coalitions shrinks to $2^{20}$, which our implementation can easily handle.

% The idea of grouping states into actors is briefly explored in the experiments in \cite{BackwardResponsibility}. However, the implementation there requires manual specification of the actors. In the following section, we explore different techniques to automatically extract actors from a reactive modules specification.


==> fix-counter.tex <==
\makeatletter

% For some reason, the envcountsame option does not work for me, so this achieves the same thing (and ensures theorem-like environments do not have an italic body)

\let\case\relax
\let\c@case\relax
\spnewtheorem{case}[theorem]{Case}{\itshape}{\rmfamily}

\let\conjecture\relax
\let\c@conjecture\relax
\spnewtheorem{conjecture}[theorem]{Conjecture}{\itshape}{\rmfamily}

\let\corollary\relax
\let\c@corollary\relax
\spnewtheorem{corollary}[theorem]{Corollary}{\bfseries}{\rmfamily}

\let\definition\relax
\let\c@definition\relax
\spnewtheorem{definition}[theorem]{Definition}{\bfseries}{\rmfamily}

\let\example\relax
\let\c@example\relax
\spnewtheorem{example}[theorem]{Example}{\itshape}{\rmfamily}

\let\exercise\relax
\let\c@exercise\relax
\spnewtheorem{exercise}[theorem]{Exercise}{\itshape}{\rmfamily}

\let\lemma\relax
\let\c@lemma\relax
\spnewtheorem{lemma}[theorem]{Lemma}{\bfseries}{\rmfamily}

\let\note\relax
\let\c@note\relax
\spnewtheorem{note}[theorem]{Note}{\itshape}{\rmfamily}

\let\problem\relax
\let\c@problem\relax
\spnewtheorem{problem}[theorem]{Problem}{\itshape}{\rmfamily}

\let\property\relax
\let\c@property\relax
\spnewtheorem{property}[theorem]{Property}{\itshape}{\rmfamily}

\let\proposition\relax
\let\c@proposition\relax
\spnewtheorem{proposition}[theorem]{Proposition}{\bfseries}{\rmfamily}

\let\question\relax
\let\c@question\relax
\spnewtheorem{question}[theorem]{Question}{\itshape}{\rmfamily}

\let\solution\relax
\let\c@solution\relax
\spnewtheorem{solution}[theorem]{Solution}{\itshape}{\rmfamily}

\let\remark\relax
\let\c@remark\relax
\spnewtheorem{remark}[theorem]{Remark}{\itshape}{\rmfamily}

\makeatother
